Towards Inferring Queries from Simple and Partial Provenance Examples

The field of query-by-example aims at inferring queries from output examples given by non-expert users, by finding the underlying logic that binds the examples. However, for a very small set of examples, it is difficult to correctly infer such logic. To bridge this gap, previous work suggested attaching explanations to each output example, modeled as provenance, allowing users to explain the reason behind their choice of example. In this paper, we explore the problem of inferring queries from a few output examples and intuitive explanations. We propose a two step framework: (1) convert the explanations into (partial) provenance and (2) infer a query that generates the output examples using a novel algorithm that employs a graph based approach. This framework is suitable for non-experts as it does not require the specification of the provenance in its entirety or an understanding of its structure. We show promising initial experimental results of our approach.

==> naive.tex <==
\paragraph*{N\"aive Approach}
Given an $(I,O)$ with full lineage provenance, the n\"aive approach would be to split this provenance set to all subsets of tuples. Suppose $I = \{t_1, \ldots, t_n\}$. Every choice of a subset from $S_1\subseteq I$ leaves $2^{|I|-|S_1|}$ options to choose the next subset of tuples $S_1\subseteq (I\setminus S_1)$. This defines a recurrence relation for the number of options to choose a subset of provenance tuple, since every tuple may be used multiple times. If $|I| = n$, $f_i = 2^{n-f_{i-1}} - 1$, where $f_n = 2^n - 1$. 
\yuval{This is not clear}
% \begin{example}
% Consider an \ex\ with a single row of provenance $\{R(1,2), R(1,3), \ldots,\}$
% \end{example}
